Scaling Experiments in Self-Supervised Cross-Table Representation Learning

To analyze the scaling potential of deep tabular representation learning models, we introduce a novel Transformer-based architecture specifically tailored to tabular data and cross-table representation learning by utilizing table-specific tokenizers and a shared Transformer backbone. Our training approach encompasses both single-table and cross-table models, trained via missing value imputation through a self-supervised masked cell recovery objective. To understand the scaling behavior of our method, we train models of varying sizes, ranging from approximately $10^4$ to $10^7$ parameters. These models are trained on a carefully curated pretraining dataset, consisting of 135M training tokens sourced from 76 diverse datasets. We assess the scaling of our architecture in both single-table and cross-table pretraining setups by evaluating the pretrained models using linear probing on a curated set of benchmark datasets and comparing the results with conventional baselines.

==> figures/0_76_datasets_information.tex <==
\begin{tabular}{lllrrrrrrr}
\toprule
                                              Name &                               Collection &       Task &  Num. Classes &  Num. rows &  Num. Cols &  Numerical Features &  Categorical Features &  Unique Categories &  NaNs (\%) \\
\midrule
                                  Brazilian\_houses &              automl\_benchmark\_regression & regression &          5751 &      10692 &         12 &                   8 &                     4 &                 44 &       0.0 \\
                                          colleges &              automl\_benchmark\_regression & regression &          4502 &       7063 &         44 &                  32 &                    12 &                206 &      33.5 \\
                                       house\_sales &              automl\_benchmark\_regression & regression &          4028 &      21613 &         21 &                  20 &                     1 &                  0 &       0.0 \\
                                         Moneyball &              automl\_benchmark\_regression & regression &           374 &       1232 &         14 &                   8 &                     6 &                 66 &      20.9 \\
                           nyc-taxi-green-dec-2016 &              automl\_benchmark\_regression & regression &          1811 &     581835 &         18 &                   9 &                     9 &                 22 &       0.0 \\
                                          2dplanes &                automl\_benchmark\_training &     binary &             2 &      40768 &         10 &                  10 &                     0 &                  0 &       0.0 \\
                                 autoUniv-au7-1100 &                automl\_benchmark\_training & multiclass &             5 &       1100 &         12 &                   8 &                     4 &                 10 &       0.0 \\
                                 BachChoralHarmony &                automl\_benchmark\_training & regression &           102 &       5665 &         16 &                   2 &                    14 &                102 &       0.0 \\
                                          bank32nh &                automl\_benchmark\_training &     binary &             2 &       8192 &         32 &                  32 &                     0 &                  0 &       0.0 \\
                                          baseball &                automl\_benchmark\_training & multiclass &             3 &       1340 &         16 &                  15 &                     1 &                  7 &       0.1 \\
                                  cardiotocography &                automl\_benchmark\_training & multiclass &            10 &       2126 &         35 &                  35 &                     0 &                  0 &       0.0 \\
                                             churn &                automl\_benchmark\_training &     binary &             2 &       5000 &         20 &                  16 &                     4 &                 17 &       0.0 \\
                                               cjs &                automl\_benchmark\_training & multiclass &             6 &       2796 &         33 &                  31 &                     2 &                 68 &      73.8 \\
                                     colleges\_aaup &                automl\_benchmark\_training &     binary &             2 &       1161 &         15 &                  13 &                     2 &                 56 &       1.5 \\
                                   colleges\_usnews &                automl\_benchmark\_training &     binary &             2 &       1302 &         33 &                  32 &                     1 &                 51 &      18.2 \\
                                  compas-two-years &                automl\_benchmark\_training &     binary &             2 &       5278 &         13 &                   7 &                     6 &                 12 &       0.0 \\
                                     Diabetes130US &                automl\_benchmark\_training & multiclass &             3 &     101766 &         49 &                  13 &                    36 &                130 &       0.0 \\
                                     eeg-eye-state &                automl\_benchmark\_training &     binary &             2 &      14980 &         14 &                  14 &                     0 &                  0 &       0.0 \\
                                         elevators &                automl\_benchmark\_training &     binary &             2 &      16599 &         18 &                  18 &                     0 &                  0 &       0.0 \\
                                     eye\_movements &                automl\_benchmark\_training & multiclass &             3 &      10936 &         27 &                  24 &                     3 &                  6 &       0.0 \\
                                              fars &                automl\_benchmark\_training & multiclass &             8 &     100968 &         29 &                  14 &                    15 &                 93 &       0.0 \\
                                             fried &                automl\_benchmark\_training &     binary &             2 &      40768 &         10 &                  10 &                     0 &                  0 &       0.0 \\
       GAMETES\_Epistasis\_3-Way\_20atts\_0.2H\_EDM-1\_1 &                automl\_benchmark\_training &     binary &             2 &       1600 &         20 &                   0 &                    20 &                 60 &       0.0 \\
GAMETES\_Heterogeneity\_20atts\_1600\_Het\_0.4\_0.2\_7... &                automl\_benchmark\_training &     binary &             2 &       1600 &         20 &                   0 &                    20 &                 59 &       0.0 \\
                 GesturePhaseSegmentationProcessed &                automl\_benchmark\_training & multiclass &             5 &       9873 &         32 &                  32 &                     0 &                  0 &       0.0 \\
                                         house\_16H &                automl\_benchmark\_training &     binary &             2 &      22784 &         16 &                  16 &                     0 &                  0 &       0.0 \\
                                       hypothyroid &                automl\_benchmark\_training & multiclass &             4 &       3772 &         29 &                   7 &                    22 &                 47 &       5.5 \\
                                    JapaneseVowels &                automl\_benchmark\_training & multiclass &             9 &       9961 &         14 &                  14 &                     0 &                  0 &       0.0 \\
                                               jm1 &                automl\_benchmark\_training &     binary &             2 &      10885 &         21 &                  21 &                     0 &                  0 &       0.0 \\
                                              kick &                automl\_benchmark\_training &     binary &             2 &      72983 &         32 &                  14 &                    18 &                134 &       6.4 \\
                                             led24 &                automl\_benchmark\_training & multiclass &            10 &       3200 &         24 &                   0 &                    24 &                 48 &       0.0 \\
                                            letter &                automl\_benchmark\_training & multiclass &            26 &      20000 &         16 &                  16 &                     0 &                  0 &       0.0 \\
                                    MagicTelescope &                automl\_benchmark\_training &     binary &             2 &      19020 &         10 &                  10 &                     0 &                  0 &       0.0 \\
                                               mc1 &                automl\_benchmark\_training &     binary &             2 &       9466 &         38 &                  38 &                     0 &                  0 &       0.0 \\
                                 microaggregation2 &                automl\_benchmark\_training & multiclass &             5 &      20000 &         20 &                  20 &                     0 &                  0 &       0.0 \\
                                       mofn-3-7-10 &                automl\_benchmark\_training &     binary &             2 &       1324 &         10 &                   0 &                    10 &                 20 &       0.0 \\
                                          mushroom &                automl\_benchmark\_training &     binary &             2 &       8124 &         22 &                   0 &                    22 &                117 &       1.4 \\
                                                mv &                automl\_benchmark\_training &     binary &             2 &      40768 &         10 &                   7 &                     3 &                  7 &       0.0 \\
                                       page-blocks &                automl\_benchmark\_training & multiclass &             5 &       5473 &         10 &                  10 &                     0 &                  0 &       0.0 \\
                                    parity5\_plus\_5 &                automl\_benchmark\_training &     binary &             2 &       1124 &         10 &                   0 &                    10 &                 20 &       0.0 \\
                                            pbcseq &                automl\_benchmark\_training &     binary &             2 &       1945 &         18 &                  12 &                     6 &                 13 &       3.2 \\
                                               pc2 &                automl\_benchmark\_training &     binary &             2 &       5589 &         36 &                  36 &                     0 &                  0 &       0.0 \\
                                         pendigits &                automl\_benchmark\_training & multiclass &            10 &      10992 &         16 &                  16 &                     0 &                  0 &       0.0 \\
                                  PhishingWebsites &                automl\_benchmark\_training &     binary &             2 &      11055 &         30 &                   0 &                    30 &                 68 &       0.0 \\
                                         pokerhand &                automl\_benchmark\_training & multiclass &            10 &     829201 &         10 &                   5 &                     5 &                 20 &       0.0 \\
                                               pol &                automl\_benchmark\_training &     binary &             2 &      15000 &         48 &                  48 &                     0 &                  0 &       0.0 \\
                                      porto-seguro &                automl\_benchmark\_training &     binary &             2 &     595212 &         37 &                  12 &                    25 &                102 &       3.8 \\
                                       qsar-biodeg &                automl\_benchmark\_training &     binary &             2 &       1055 &         41 &                  41 &                     0 &                  0 &       0.0 \\
                                          ringnorm &                automl\_benchmark\_training &     binary &             2 &       7400 &         20 &                  20 &                     0 &                  0 &       0.0 \\
                                                rl &                automl\_benchmark\_training &     binary &             2 &      31406 &         22 &                   8 &                    14 &                 89 &       4.3 \\
                                          satimage &                automl\_benchmark\_training & multiclass &             6 &       6430 &         36 &                  36 &                     0 &                  0 &       0.0 \\
                               spoken-arabic-digit &                automl\_benchmark\_training & multiclass &            10 &     263256 &         14 &                  14 &                     0 &                  0 &       0.0 \\
                                steel-plates-fault &                automl\_benchmark\_training &     binary &             2 &       1941 &         33 &                  33 &                     0 &                  0 &       0.0 \\
                                           texture &                automl\_benchmark\_training & multiclass &            11 &       5500 &         40 &                  40 &                     0 &                  0 &       0.0 \\
                                Traffic\_violations &                automl\_benchmark\_training & multiclass &             3 &      70340 &         20 &                   1 &                    19 &                268 &       0.2 \\
                             wall-robot-navigation &                automl\_benchmark\_training & multiclass &             4 &       5456 &         24 &                  24 &                     0 &                  0 &       0.0 \\
                                     waveform-5000 &                automl\_benchmark\_training & multiclass &             3 &       5000 &         40 &                  40 &                     0 &                  0 &       0.0 \\
                                              wind &                automl\_benchmark\_training &     binary &             2 &       6574 &         14 &                  14 &                     0 &                  0 &       0.0 \\
                                  wine-quality-red &                automl\_benchmark\_training & multiclass &             6 &       1599 &         11 &                  11 &                     0 &                  0 &       0.0 \\
                                wine-quality-white &                automl\_benchmark\_training & multiclass &             7 &       4898 &         11 &                  11 &                     0 &                  0 &       0.0 \\
                                      cpu\_activity &                             openml\_ctr23 & regression &            56 &       8192 &         21 &                  21 &                     0 &                  0 &       0.0 \\
                                              fifa &                             openml\_ctr23 & regression &           133 &      19178 &         28 &                  27 &                     1 &                  0 &       0.0 \\
                                     fps\_benchmark &                             openml\_ctr23 & regression &          2675 &      24624 &         43 &                  30 &                    13 &                 96 &       6.6 \\
                                    grid\_stability &                             openml\_ctr23 & regression &         10000 &      10000 &         12 &                  12 &                     0 &                  0 &       0.0 \\
                                  health\_insurance &                             openml\_ctr23 & regression &            75 &      22272 &         11 &                   4 &                     7 &                 21 &       0.0 \\
                                      kings\_county &                             openml\_ctr23 & regression &          4028 &      21613 &         21 &                  17 &                     4 &                 45 &       0.0 \\
                                     miami\_housing &                             openml\_ctr23 & regression &          2111 &      13932 &         15 &                  15 &                     0 &                  0 &       0.0 \\
                            naval\_propulsion\_plant &                             openml\_ctr23 & regression &            51 &      11934 &         14 &                  14 &                     0 &                  0 &       0.0 \\
                                       pumadyn32nh &                             openml\_ctr23 & regression &          8191 &       8192 &         32 &                  32 &                     0 &                  0 &       0.0 \\
                                            sarcos &                             openml\_ctr23 & regression &         11414 &      48933 &         21 &                  21 &                     0 &                  0 &       0.0 \\
                                       solar\_flare &                             openml\_ctr23 & multiclass &             8 &       1066 &         10 &                   2 &                     8 &                 27 &       0.0 \\
                                 video\_transcoding &                             openml\_ctr23 & regression &         10960 &      68784 &         18 &                  16 &                     2 &                  8 &       0.0 \\
                                       wave\_energy &                             openml\_ctr23 & regression &         71993 &      72000 &         48 &                  48 &                     0 &                  0 &       0.0 \\
                               Bike\_Sharing\_Demand & tabular\_benchmark\_categorical\_regression & regression &           869 &      17379 &         11 &                   6 &                     5 &                 14 &       0.0 \\
                           delays\_zurich\_transport & tabular\_benchmark\_categorical\_regression & regression &          4082 &    5465575 &         11 &                   8 &                     3 &                 12 &       0.0 \\
                                          Ailerons &   tabular\_benchmark\_numerical\_regression & multiclass &            35 &      13750 &         33 &                  33 &                     0 &                  0 &       0.0 \\
\bottomrule
\end{tabular}


==> tables/0_76_datasets_information.tex <==
\begin{tabular}{lllrrrrrrr}
\toprule
                                              Name &                               Collection &       Task &  Num. Classes &  Num. rows &  Num. Cols &  Numerical Features &  Categorical Features &  Unique Categories &  NaNs (\%) \\
\midrule
                                  Brazilian\_houses &              automl\_benchmark\_regression & regression &          5751 &      10692 &         12 &                   8 &                     4 &                 44 &       0.0 \\
                                          colleges &              automl\_benchmark\_regression & regression &          4502 &       7063 &         44 &                  32 &                    12 &                206 &      33.5 \\
                                       house\_sales &              automl\_benchmark\_regression & regression &          4028 &      21613 &         21 &                  20 &                     1 &                  0 &       0.0 \\
                                         Moneyball &              automl\_benchmark\_regression & regression &           374 &       1232 &         14 &                   8 &                     6 &                 66 &      20.9 \\
                           nyc-taxi-green-dec-2016 &              automl\_benchmark\_regression & regression &          1811 &     581835 &         18 &                   9 &                     9 &                 22 &       0.0 \\
                                          2dplanes &                automl\_benchmark\_training &     binary &             2 &      40768 &         10 &                  10 &                     0 &                  0 &       0.0 \\
                                 autoUniv-au7-1100 &                automl\_benchmark\_training & multiclass &             5 &       1100 &         12 &                   8 &                     4 &                 10 &       0.0 \\
                                 BachChoralHarmony &                automl\_benchmark\_training & regression &           102 &       5665 &         16 &                   2 &                    14 &                102 &       0.0 \\
                                          bank32nh &                automl\_benchmark\_training &     binary &             2 &       8192 &         32 &                  32 &                     0 &                  0 &       0.0 \\
                                          baseball &                automl\_benchmark\_training & multiclass &             3 &       1340 &         16 &                  15 &                     1 &                  7 &       0.1 \\
                                  cardiotocography &                automl\_benchmark\_training & multiclass &            10 &       2126 &         35 &                  35 &                     0 &                  0 &       0.0 \\
                                             churn &                automl\_benchmark\_training &     binary &             2 &       5000 &         20 &                  16 &                     4 &                 17 &       0.0 \\
                                               cjs &                automl\_benchmark\_training & multiclass &             6 &       2796 &         33 &                  31 &                     2 &                 68 &      73.8 \\
                                     colleges\_aaup &                automl\_benchmark\_training &     binary &             2 &       1161 &         15 &                  13 &                     2 &                 56 &       1.5 \\
                                   colleges\_usnews &                automl\_benchmark\_training &     binary &             2 &       1302 &         33 &                  32 &                     1 &                 51 &      18.2 \\
                                  compas-two-years &                automl\_benchmark\_training &     binary &             2 &       5278 &         13 &                   7 &                     6 &                 12 &       0.0 \\
                                     Diabetes130US &                automl\_benchmark\_training & multiclass &             3 &     101766 &         49 &                  13 &                    36 &                130 &       0.0 \\
                                     eeg-eye-state &                automl\_benchmark\_training &     binary &             2 &      14980 &         14 &                  14 &                     0 &                  0 &       0.0 \\
                                         elevators &                automl\_benchmark\_training &     binary &             2 &      16599 &         18 &                  18 &                     0 &                  0 &       0.0 \\
                                     eye\_movements &                automl\_benchmark\_training & multiclass &             3 &      10936 &         27 &                  24 &                     3 &                  6 &       0.0 \\
                                              fars &                automl\_benchmark\_training & multiclass &             8 &     100968 &         29 &                  14 &                    15 &                 93 &       0.0 \\
                                             fried &                automl\_benchmark\_training &     binary &             2 &      40768 &         10 &                  10 &                     0 &                  0 &       0.0 \\
       GAMETES\_Epistasis\_3-Way\_20atts\_0.2H\_EDM-1\_1 &                automl\_benchmark\_training &     binary &             2 &       1600 &         20 &                   0 &                    20 &                 60 &       0.0 \\
GAMETES\_Heterogeneity\_20atts\_1600\_Het\_0.4\_0.2\_7... &                automl\_benchmark\_training &     binary &             2 &       1600 &         20 &                   0 &                    20 &                 59 &       0.0 \\
                 GesturePhaseSegmentationProcessed &                automl\_benchmark\_training & multiclass &             5 &       9873 &         32 &                  32 &                     0 &                  0 &       0.0 \\
                                         house\_16H &                automl\_benchmark\_training &     binary &             2 &      22784 &         16 &                  16 &                     0 &                  0 &       0.0 \\
                                       hypothyroid &                automl\_benchmark\_training & multiclass &             4 &       3772 &         29 &                   7 &                    22 &                 47 &       5.5 \\
                                    JapaneseVowels &                automl\_benchmark\_training & multiclass &             9 &       9961 &         14 &                  14 &                     0 &                  0 &       0.0 \\
                                               jm1 &                automl\_benchmark\_training &     binary &             2 &      10885 &         21 &                  21 &                     0 &                  0 &       0.0 \\
                                              kick &                automl\_benchmark\_training &     binary &             2 &      72983 &         32 &                  14 &                    18 &                134 &       6.4 \\
                                             led24 &                automl\_benchmark\_training & multiclass &            10 &       3200 &         24 &                   0 &                    24 &                 48 &       0.0 \\
                                            letter &                automl\_benchmark\_training & multiclass &            26 &      20000 &         16 &                  16 &                     0 &                  0 &       0.0 \\
                                    MagicTelescope &                automl\_benchmark\_training &     binary &             2 &      19020 &         10 &                  10 &                     0 &                  0 &       0.0 \\
                                               mc1 &                automl\_benchmark\_training &     binary &             2 &       9466 &         38 &                  38 &                     0 &                  0 &       0.0 \\
                                 microaggregation2 &                automl\_benchmark\_training & multiclass &             5 &      20000 &         20 &                  20 &                     0 &                  0 &       0.0 \\
                                       mofn-3-7-10 &                automl\_benchmark\_training &     binary &             2 &       1324 &         10 &                   0 &                    10 &                 20 &       0.0 \\
                                          mushroom &                automl\_benchmark\_training &     binary &             2 &       8124 &         22 &                   0 &                    22 &                117 &       1.4 \\
                                                mv &                automl\_benchmark\_training &     binary &             2 &      40768 &         10 &                   7 &                     3 &                  7 &       0.0 \\
                                       page-blocks &                automl\_benchmark\_training & multiclass &             5 &       5473 &         10 &                  10 &                     0 &                  0 &       0.0 \\
                                    parity5\_plus\_5 &                automl\_benchmark\_training &     binary &             2 &       1124 &         10 &                   0 &                    10 &                 20 &       0.0 \\
                                            pbcseq &                automl\_benchmark\_training &     binary &             2 &       1945 &         18 &                  12 &                     6 &                 13 &       3.2 \\
                                               pc2 &                automl\_benchmark\_training &     binary &             2 &       5589 &         36 &                  36 &                     0 &                  0 &       0.0 \\
                                         pendigits &                automl\_benchmark\_training & multiclass &            10 &      10992 &         16 &                  16 &                     0 &                  0 &       0.0 \\
                                  PhishingWebsites &                automl\_benchmark\_training &     binary &             2 &      11055 &         30 &                   0 &                    30 &                 68 &       0.0 \\
                                         pokerhand &                automl\_benchmark\_training & multiclass &            10 &     829201 &         10 &                   5 &                     5 &                 20 &       0.0 \\
                                               pol &                automl\_benchmark\_training &     binary &             2 &      15000 &         48 &                  48 &                     0 &                  0 &       0.0 \\
                                      porto-seguro &                automl\_benchmark\_training &     binary &             2 &     595212 &         37 &                  12 &                    25 &                102 &       3.8 \\
                                       qsar-biodeg &                automl\_benchmark\_training &     binary &             2 &       1055 &         41 &                  41 &                     0 &                  0 &       0.0 \\
                                          ringnorm &                automl\_benchmark\_training &     binary &             2 &       7400 &         20 &                  20 &                     0 &                  0 &       0.0 \\
                                                rl &                automl\_benchmark\_training &     binary &             2 &      31406 &         22 &                   8 &                    14 &                 89 &       4.3 \\
                                          satimage &                automl\_benchmark\_training & multiclass &             6 &       6430 &         36 &                  36 &                     0 &                  0 &       0.0 \\
                               spoken-arabic-digit &                automl\_benchmark\_training & multiclass &            10 &     263256 &         14 &                  14 &                     0 &                  0 &       0.0 \\
                                steel-plates-fault &                automl\_benchmark\_training &     binary &             2 &       1941 &         33 &                  33 &                     0 &                  0 &       0.0 \\
                                           texture &                automl\_benchmark\_training & multiclass &            11 &       5500 &         40 &                  40 &                     0 &                  0 &       0.0 \\
                                Traffic\_violations &                automl\_benchmark\_training & multiclass &             3 &      70340 &         20 &                   1 &                    19 &                268 &       0.2 \\
                             wall-robot-navigation &                automl\_benchmark\_training & multiclass &             4 &       5456 &         24 &                  24 &                     0 &                  0 &       0.0 \\
                                     waveform-5000 &                automl\_benchmark\_training & multiclass &             3 &       5000 &         40 &                  40 &                     0 &                  0 &       0.0 \\
                                              wind &                automl\_benchmark\_training &     binary &             2 &       6574 &         14 &                  14 &                     0 &                  0 &       0.0 \\
                                  wine-quality-red &                automl\_benchmark\_training & multiclass &             6 &       1599 &         11 &                  11 &                     0 &                  0 &       0.0 \\
                                wine-quality-white &                automl\_benchmark\_training & multiclass &             7 &       4898 &         11 &                  11 &                     0 &                  0 &       0.0 \\
                                      cpu\_activity &                             openml\_ctr23 & regression &            56 &       8192 &         21 &                  21 &                     0 &                  0 &       0.0 \\
                                              fifa &                             openml\_ctr23 & regression &           133 &      19178 &         28 &                  27 &                     1 &                  0 &       0.0 \\
                                     fps\_benchmark &                             openml\_ctr23 & regression &          2675 &      24624 &         43 &                  30 &                    13 &                 96 &       6.6 \\
                                    grid\_stability &                             openml\_ctr23 & regression &         10000 &      10000 &         12 &                  12 &                     0 &                  0 &       0.0 \\
                                  health\_insurance &                             openml\_ctr23 & regression &            75 &      22272 &         11 &                   4 &                     7 &                 21 &       0.0 \\
                                      kings\_county &                             openml\_ctr23 & regression &          4028 &      21613 &         21 &                  17 &                     4 &                 45 &       0.0 \\
                                     miami\_housing &                             openml\_ctr23 & regression &          2111 &      13932 &         15 &                  15 &                     0 &                  0 &       0.0 \\
                            naval\_propulsion\_plant &                             openml\_ctr23 & regression &            51 &      11934 &         14 &                  14 &                     0 &                  0 &       0.0 \\
                                       pumadyn32nh &                             openml\_ctr23 & regression &          8191 &       8192 &         32 &                  32 &                     0 &                  0 &       0.0 \\
                                            sarcos &                             openml\_ctr23 & regression &         11414 &      48933 &         21 &                  21 &                     0 &                  0 &       0.0 \\
                                       solar\_flare &                             openml\_ctr23 & multiclass &             8 &       1066 &         10 &                   2 &                     8 &                 27 &       0.0 \\
                                 video\_transcoding &                             openml\_ctr23 & regression &         10960 &      68784 &         18 &                  16 &                     2 &                  8 &       0.0 \\
                                       wave\_energy &                             openml\_ctr23 & regression &         71993 &      72000 &         48 &                  48 &                     0 &                  0 &       0.0 \\
                               Bike\_Sharing\_Demand & tabular\_benchmark\_categorical\_regression & regression &           869 &      17379 &         11 &                   6 &                     5 &                 14 &       0.0 \\
                           delays\_zurich\_transport & tabular\_benchmark\_categorical\_regression & regression &          4082 &    5465575 &         11 &                   8 &                     3 &                 12 &       0.0 \\
                                          Ailerons &   tabular\_benchmark\_numerical\_regression & multiclass &            35 &      13750 &         33 &                  33 &                     0 &                  0 &       0.0 \\
\bottomrule
\end{tabular}

